Documentation-as-code for Interface Control Document Management in Systems of Systems: a Technical Action Research Study

The architecting of Systems of Systems (SoS), that is, of systems that emerge from the cooperation of multiple independent constituent systems, is a topic of increasing interest in both industry and academia. However, recent empirical studies revealed what seems to be an overlooked aspect of the architecting of SoS that is linked to major integration and operational issues: the interplay between the various disciplines involved in such an architecting process. This aspect becomes particularly relevant for the management of the interfaces between the SoS constituents, where such disciplines inevitably meet. In this paper, we present the results of the first cycle of a Technical Action Research (TAR) study conducted in cooperation between the authors and a group of practitioners involved in the long-running architecting process of a large-scale radio astronomy SoS project. This TAR is aimed at exploring potential improvements of the document-centered interface management approach currently followed in this project by adopting elements of the \textit{documentation-as-code} philosophy, which is widely adopted in the domain of software systems. As a result, a working proof-of-concept of an ICD (Interface Control Document) management approach was developed by the researchers and evaluated by the practitioners. The results of the study and the corresponding lessons learned are reported in this work.

==> detemplatelisting.tex <==
\lstinputlisting[language=JavaScript, 
caption=Data extraction from \cite{gillies_database_2016}
]{datac/guilles.js}

\lstinputlisting[language=JavaScript, 
caption=Data extraction from \cite{vipavetz_interface_2016}
]{datac/vipavetz.js}

\lstinputlisting[language=JavaScript, 
caption=Data extraction from \cite{borrowman_can_2016}
]{datac/borrowman.js}


==> jslistings.tex <==
\lstdefinelanguage{CSS}{
  keywords={color,background-image:,margin,padding,font,weight,display,position,top,left,right,bottom,list,style,border,size,white,space,min,width, transition:, transform:, transition-property, transition-duration, transition-timing-function},	
  sensitive=true,
  morecomment=[l]{//},
  morecomment=[s]{/*}{*/},
  morestring=[b]',
  morestring=[b]",
  alsoletter={:},
  alsodigit={-}
}

\lstdefinelanguage{JavaScript}{
  morekeywords={typeof, new, true, false, catch, function, return, null, catch, switch, var, if, in, while, do, else, case, break},
  morecomment=[s]{/*}{*/},
  morecomment=[l]//,
  morestring=[b]",
  morestring=[b]'
}

\lstdefinelanguage{HTML5}{
  language=html,
  sensitive=true,	
  alsoletter={<>=-},	
  morecomment=[s]{<!-}{-->},
  tag=[s],
  otherkeywords={
  >,
	<!DOCTYPE,
  </html, <html, <head, <title, </title, <style, </style, <link, </head, <meta, />,
	</body, <body,
	</div, <div, </div>, 
	</p, <p, </p>,
	</script, <script,
  <canvas, /canvas>, <svg, <rect, <animateTransform, </rect>, </svg>, <video, <source, <iframe, </iframe>, </video>, <image, </image>, <header, </header, <article, </article
  },
  ndkeywords={
  =,
  charset=, src=, id=, width=, height=, style=, type=, rel=, href=,
  fill=, attributeName=, begin=, dur=, from=, to=, poster=, controls=, x=, y=, repeatCount=, xlink:href=,
  margin:, padding:, background-image:, border:, top:, left:, position:, width:, height:, margin-top:, margin-bottom:, font-size:, line-height:,
  transform:, -moz-transform:, -webkit-transform:,
  animation:, -webkit-animation:,
  transition:,  transition-duration:, transition-property:, transition-timing-function:,
  }
}

\lstdefinestyle{htmlcssjs} {%
  basicstyle={\footnotesize\ttfamily},   
  frame=b,
  xleftmargin={0.75cm},
  numbers=left,
  stepnumber=1,
  firstnumber=1,
  numberfirstline=true,	
  identifierstyle=\color{black},
  keywordstyle=\color{blue}\bfseries,
  ndkeywordstyle=\color{editorGreen}\bfseries,
  stringstyle=\color{editorOcher}\ttfamily,
  commentstyle=\color{brown}\ttfamily,
  language=HTML5,
  alsolanguage=JavaScript,
  alsodigit={.:;},	
  tabsize=2,
  showtabs=false,
  showspaces=false,
  showstringspaces=false,
  extendedchars=true,
  breaklines=true,
  literate=%
  {Ö}{{\"O}}1
  {Ä}{{\"A}}1
  {Ü}{{\"U}}1
  {ß}{{\ss}}1
  {ü}{{\"u}}1
  {ä}{{\"a}}1
  {ö}{{\"o}}1
}

==> related_w.tex <==

ICDs usually differ substantially from one company to another~\cite{rahmani_managing_2011}, even within the same application domain~\cite{louadah_towards_2014}, and the approaches for managing them, depend on whether the project follows a document-based (DBSE) or model-based (MBSE) systems engineering approach. In the former, the ICDs capture design information in textual format. In the latter, where formal domain models are used as the central element of the process (to avoid some the limitations of the document-centered one), the ICDs, when needed, are automatically generated from the latest version of such formal model (e.g., ~\cite{gillies_database_2016,borrowman_can_2016,zheng_multidisciplinary_2017,rahmani_ontology_2012,ps_interface_2015}). The documentation approach explored in this study is aimed at SoS projects that follow a document-centered approach --still a widely used one~ \cite{broy2021advanced}-- like LOFAR.
\todo[inline]{WIP}

==> research_problem.tex <==
The main goal of this study is to investigate an alternative interface management approach that could improve misunderstandings and the need for assumptions while working with interface specifications (i.e., with ICDs). More specifically, this study aims to explore to what extent this alternative interface management approach could improve the documentation qualities that, according to recent empirical studies~\cite{cadavidsurvey,cadavid2021system}, are related to the aforementioned misunderstanding and assumptions-related issues, namely: \textit{completeness}, \textit{uniformity}, \textit{clarity}, and \textit{understandability across domains}. During the formulation of the action research study, it was agreed by the researchers and ASTRON participants to scope the first cycle of the study to a management approach based on the \textit{DaC} philosophy. The rationale for this was two-fold: first, the researchers had already identified that the potential features of an ICD \textit{DaC}-pipeline would seemingly address the aforementioned qualities to be addressed, as summarized in Table~\ref{tab:dac-features-vs-qualities}. Second, ASTRON participants agreed to explore this approach, as they had already been exploring approaches to reliably generate documentation and software artifacts from human-readable text-based specifications.

\begin{table}[h]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{Xccc}
		\toprule
		\textbf{Quality/DaC feature} & \textbf{Collaboration} & \textbf{Automated validation} & \textbf{Content generation} \\ 
		\hline
		Completeness & X & X  & \\
		\hline
		Clarity & X & X &  \\
		\hline
		Uniformity &  & X & X \\
		\hline
		Cross-domain understandability & X & X & X \\
		\bottomrule
	\end{tabularx}
	
	\caption{\label{tab:dac-features-vs-qualities}The completeness and clarity of the documents could be improved by being both human and machine-readable. With the former, and using the collaboration features of modern version control systems (e.g., issues trackers), these features can be improved (or at least kept as is) by means of human cooperation. By being machine-readable, on other hand, completeness and clarity could be further improved by means of automated quality assessments. When it comes to uniformity on ICDs, that could be improved by means of content generators, as these would define standardized templates to be used across the documentation in the system. Finally, the cross-domain understandability of the ICDs could be improved not only through human cooperation, but by automatically validating the existence of misinterpretation-prone elements, and by automatically generating sections with the information required for a proper understanding of said document.}	
\end{table}

Consequently, a DaC pipeline \textit{proof-of-concept} tailored to the context of ICDs in a SoS, and focused on hardware-software interface descriptions, was designed and evaluated as a \textit{treatment} for the ICDs issues discussed above. Therefore, the goal of this study can be described following the \textit{design problem} structure proposed by Wieringa~\cite{wieringa2014design}, and a series of research questions as follows:

\begin{framed}
	\begin{quote}
		\textbf{Improve} completeness, uniformity, clarity, and cross-domain understandability of ICDs.\\
		\textbf{By} adapting DaC principles into hardware/software ICDs management\\
		\textbf{Such that} the documents created following this approach lead to less assumptions and misunderstandings while working with them\\
		\textbf{In order to} reduce potential integration and operational issues caused by them.
	\end{quote}
\end{framed}

\begin{description}
	\item[RQ1] What are the requirements for a \textit{DaC} ICD management workflow for hardware/software interfaces to improve their completeness, uniformity, clarity, and cross-domain understandability?
	\item[RQ2] What is the design of a DaC-based documentation workflow and document structure to address the identified requirements? \textit{This research issue focuses on the prototype implementation and conceptual evaluation.}	
	\item[RQ3] To what extent the designed documentation management approach would improve completeness, uniformity, clarity, and cross-domain understandability issues?
\end{description}


